LILAC: Log Parsing using LLMs with Adaptive Parsing Cache

Log parsing transforms log messages into structured formats, serving as the prerequisite step for various log analysis tasks. Although a variety of log parsing approaches have been proposed, their performance on complicated log data remains compromised due to the use of human-crafted rules or learning-based models with limited training data. The recent emergence of powerful large language models (LLMs) demonstrates their vast pre-trained knowledge related to code and logging, making it promising to apply LLMs for log parsing. However, their lack of specialized log parsing capabilities currently hinders their accuracy in parsing. Moreover, the inherent inconsistent answers, as well as the substantial overhead, prevent the practical adoption of LLM-based log parsing. To address these challenges, we propose LILAC, the first practical log parsing framework using LLMs with adaptive parsing cache. To facilitate accurate and robust log parsing, LILAC leverages the in-context learning (ICL) capability of the LLM by performing a hierarchical candidate sampling algorithm and selecting high-quality demonstrations. Furthermore, LILAC incorporates a novel component, an adaptive parsing cache, to store and refine the templates generated by the LLM. It helps mitigate LLM's inefficiency issue by enabling rapid retrieval of previously processed log templates. In this process, LILAC adaptively updates the templates within the parsing cache to ensure the consistency of parsed results. The extensive evaluation on public large-scale datasets shows that LILAC outperforms state-of-the-art methods by 69.5% in terms of the average F1 score of template accuracy. In addition, LILAC reduces the query times to LLMs by several orders of magnitude, achieving a comparable efficiency to the fastest baseline.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Tables/RQ1-bp.tex <==
\begin{table*}[]
\captionsetup{justification=centering}
\centering
\caption{Accuracy comparison between baselines and \nm with 32-shot on public datasets}
\label{tab: RQ1}
%\vspace{-12pt}
 \resizebox{\textwidth}{!}{%\
\begin{tabular}{c|cccc|cccc|cccc|cccc|cccc}
% \begin{tabular}{c|lllllllllllllllllllllllllllll}
\toprule
\  & \multicolumn{4}{c|}{AEL} & \multicolumn{4}{c|}{Drain} & \multicolumn{4}{c|}{UniParser} & \multicolumn{4}{c|}{LogPPT} & \multicolumn{4}{c}{\nm} \\
\  & GA & FGA & PA & FTA & GA & FGA & PA & FTA & GA & FGA & PA & FTA & GA & FGA & PA & FTA & GA & FGA & PA & FTA \\
\hline
Hadoop & 0.823 & 0.117 & 0.535 & 0.058 & 0.921 & 0.785 & 0.541 & 0.384 & 0.691 & 0.628 & 0.889 & 0.476 & 0.483 & 0.526 & 0.666 & 0.434 & 0.872 & 0.962 & 0.832 & 0.779 \\ 
HDFS & 0.999 & 0.764 & 0.621 & 0.562 & 0.999 & 0.935 & 0.621 & 0.609 & 1.000 & 0.968 & 0.948 & 0.581 & 0.721 & 0.391 & 0.943 & 0.312 & 1.000 & 0.968 & 0.999 & 0.946 \\ 
OpenStack & 0.743 & 0.682 & 0.029 & 0.165 & 0.752 & 0.007 & 0.029 & 0.002 & 1.000 & 0.969 & 0.516 & 0.289 & 0.534 & 0.874 & 0.406 & 0.738 & 1.000 & 1.000 & 1.000 & 0.979 \\ 
Spark & --- & --- & --- & --- & 0.888 & 0.861 & 0.394 & 0.412 & 0.854 & 0.020 & 0.795 & 0.012 & 0.476 & 0.374 & 0.952 & 0.299 & 1.000 & 0.901 & 0.973 & 0.759 \\ 
Zookeeper & 0.996 & 0.788 & 0.842 & 0.465 & 0.994 & 0.904 & 0.843 & 0.614 & 0.988 & 0.661 & 0.988 & 0.510 & 0.967 & 0.918 & 0.845 & 0.809 & 1.000 & 0.967 & 0.687 & 0.868 \\ 
BGL & 0.915 & 0.587 & 0.406 & 0.165 & 0.919 & 0.624 & 0.407 & 0.193 & 0.918 & 0.624 & 0.949 & 0.219 & 0.245 & 0.253 & 0.938 & 0.261 & 0.894 & 0.859 & 0.958 & 0.746 \\ 
HPC & 0.748 & 0.201 & 0.741 & 0.136 & 0.793 & 0.309 & 0.721 & 0.152 & 0.777 & 0.660 & 0.941 & 0.351 & 0.782 & 0.780 & 0.997 & 0.768 & 0.869 & 0.907 & 0.705 & 0.800 \\ 
Thunderbird & 0.786 & 0.116 & 0.163 & 0.035 & 0.831 & 0.237 & 0.216 & 0.071 & 0.579 & 0.682 & 0.654 & 0.290 & 0.564 & 0.216 & 0.401 & 0.117 & 0.806 & 0.793 & 0.559 & 0.572 \\ 
Linux & 0.916 & 0.806 & 0.082 & 0.217 & 0.686 & 0.778 & 0.111 & 0.259 & 0.285 & 0.451 & 0.164 & 0.232 & 0.205 & 0.712 & 0.168 & 0.428 & 0.971 & 0.931 & 0.765 & 0.740 \\ 
Mac & 0.797 & 0.793 & 0.245 & 0.205 & 0.761 & 0.229 & 0.357 & 0.069 & 0.737 & 0.699 & 0.688 & 0.283 & 0.544 & 0.493 & 0.390 & 0.274 & 0.876 & 0.825 & 0.638 & 0.553 \\ 
Apache & 1.000 & 1.000 & 0.727 & 0.517 & 1.000 & 1.000 & 0.727 & 0.517 & 0.948 & 0.687 & 0.942 & 0.269 & 0.786 & 0.605 & 0.948 & 0.368 & 1.000 & 1.000 & 0.996 & 0.862 \\ 
OpenSSH & 0.705 & 0.689 & 0.364 & 0.333 & 0.707 & 0.872 & 0.586 & 0.487 & 0.275 & 0.009 & 0.289 & 0.005 & 0.277 & 0.081 & 0.654 & 0.105 & 0.690 & 0.838 & 0.941 & 0.865 \\ 
HealthApp & 0.725 & 0.008 & 0.311 & 0.003 & 0.862 & 0.010 & 0.312 & 0.004 & 0.461 & 0.745 & 0.817 & 0.462 & 0.998 & 0.947 & 0.997 & 0.822 & 1.000 & 0.981 & 0.729 & 0.873 \\ 
Proxifier & 0.974 & 0.667 & 0.677 & 0.417 & 0.692 & 0.206 & 0.688 & 0.176 & 0.509 & 0.286 & 0.634 & 0.457 & 0.989 & 0.870 & 1.000 & 0.957 & 1.000 & 1.000 & 1.000 & 1.000 \\ 
\hline
Average & 0.856 & 0.555 & 0.442 & 0.252 & 0.843 & 0.554 & 0.468 & 0.282 & 0.716 & 0.578 & 0.730 & 0.317 & 0.612 & 0.574 & 0.736 & 0.478 & 0.927 & 0.924 & 0.842 & 0.810 \\ 
\bottomrule
\end{tabular}
}
\end{table*}





==> Tables/RQ2-coverage.tex <==
\begin{table*}[htbp]
\captionsetup{justification=centering}
\centering
\caption{Average sampling coverage comparison between algorithms of \nm and LogPPT on public datasets}
\label{tab: RQ3-coverage}
%\vspace{-12pt}
 \resizebox{0.75\textwidth}{!}{%\
\begin{tabular}{lccccc}
\toprule
 & 8 candidates & 16 candidates & 32 candidates & 64 candidates & 128 candidates\\
 \hline
LogPPT & 97.3\% & 94.0\% & 88.1\% & 83.0\% & 76.8\% \\
\nm & 98.2\% ($\uparrow 0.9\%$) & 98.0\% ($\uparrow 4.3\%$) & 96.6\% ($\uparrow 9.6\%$)& 93.7\% ($\uparrow 12.9\%$) & 92.2\% ($\uparrow 20.1\%$)\\
\bottomrule
\end{tabular}
}
\end{table*}

==> Tables/RQ4-parsing_efficiency.tex <==
\vspace{-10pt}
\begin{table*}[htbp]
\captionsetup{justification=centering}
\centering
\caption{Parsing time of baselines and \nm with different LLMs on public datasets (seconds)}
\label{tab: RQ4_parsing}
\vspace{-12pt}
 \resizebox{0.7\textwidth}{!}{ %\
\begin{tabular}{c|cccc|ccc}
% \begin{tabular}{c|lllllllllllllllllllllllllllll}
\toprule
% \multirow{2}{*}{}  & \multirow{2}{*}{AEL} & \multirow{2}{*}{Drain} & \multirow{2}{*}{UniParser} & \multirow{2}{*}{LogPPT} & \multirow{2}{*}{\nm} & \multirow{2}{*}{\makecell{process time}} & \multirow{2}{*}{\makecell{query time}} \\
 & AEL & Drain & UniParser & LogPPT & \nm & cache operation & query \\
\hline
% Proxifier & 21,320 & 11 & 1.4 & 2.9 & 14.7 & 22.8 & 12.7 \\ 
% Linux & 23,921 & 338 & 3.9 & 2.6 & 10.1 & 18.6 & 266.5 \\
% Apache & 51,977 & 29 & 2.7 & 5.1 & 21.0 & 35.1 & 28.6 \\
% Zookeeper & 74,273 & 89 & 2.8 & 7.0 & 50.6 & 49.5 & 75.9 \\
% Mac & 100,314 & 626 & 8.6 & 17.0 & 67.0 & 193.7 & 1040.8 \\
% OpenStack & 207,632 & 48 & 25.7 & 64.3 & 138.7 & 371.7 & 60.8 \\
% HealthApp & 212,394 & 156 & 349.5 & 17.7 & 71.4 & 170.1 & 103.4 \\ 
% Hadoop & 179,993 & 236 & 83.1 & 19.3 & 83.3 & 191.4 & 213.6 \\
% HPC & 429,987 & 74 & 15.1 & 37.8 & 109.0 & 219.1 & 93.4 \\
% OpenSSH & 638,946 & 38 & 344.1 & 74.1 & 328.3 & 671.5 & 78.2 \\
% BGL & 4,631,261 & 320 & 9269.8 & 498.3 & 1685.3 & 2456.4 & 1060.9 \\
% HDFS & 11,167,740 & 46 & 1403.0 & 1123.3 & 4819.0 & 12133.7 & 836.7 \\
% Spark & 16,075,117 & 236 & ---- &  1593.8 & 8806.8 & 13995.6 & 1190.1 \\
% Thunderbird & 16,601,745 & 1241 & 11807.5 & 2491.8 & 15368.4 & 27008.6 &  2913.4 \\
% \hline
Average time & 1793.6 & 425.4 & 2293.8 & 4097.6 & 569.6 & 376.5 & 193.1 \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table*}

==> Tables/RQ4-parsing_efficiency_bp.tex <==
\begin{table*}[]
\captionsetup{justification=centering}
\centering
\caption{Detailed parsing time of baselines and \nm on public datasets (seconds)}
\label{tab: RQ4_parsing}
%\vspace{-12pt}
 \resizebox{\textwidth}{!}{ %\
\begin{tabular}{ccc|ccccc}
% \begin{tabular}{c|lllllllllllllllllllllllllll}
\toprule
\multirow{2}{*}{Datasets} & \multirow{2}{*}{\# Log} & \multirow{2}{*}{\# Temp.} & \multirow{2}{*}{AEL} & \multirow{2}{*}{Drain} & \multirow{2}{*}{UniParser} & \multirow{2}{*}{LogPPT}  & \multirow{2}{*}{\nm} & \multirow{2}{*} \\
 & & & & & & & &
\hline
Proxifier & 21,320 & 11 & 1.4 & 2.9 & 14.7 & 22.8 &  12.7 \\ 
Linux & 23,921 & 338 & 3.9 & 2.6 & 10.1 & 18.6 & 266.5  \\
Apache & 51,977 & 29 & 2.7 & 5.1 & 21.0 & 35.1 & 28.6  \\
Zookeeper & 74,273 & 89 & 2.8 & 7.0 & 50.6 & 49.5 &  75.9  \\
Mac & 100,314 & 626 & 8.6 & 17.0 & 67.0 & 193.7 &  1040.8  \\
OpenStack & 207,632 & 48 & 25.7 & 64.3 & 138.7 & 371.7 &  60.8  \\
HealthApp & 212,394 & 156 & 349.5 & 17.7 & 71.4 & 170.1 &  103.4  \\ 
Hadoop & 179,993 & 236 & 83.1 & 19.3 & 83.3 & 191.4 & 213.6  \\
HPC & 429,987 & 74 & 15.1 & 37.8 & 109.0 & 219.1 &  93.4  \\
OpenSSH & 638,946 & 38 & 344.1 & 74.1 & 328.3 & 671.5 &  78.2  \\
BGL & 4,631,261 & 320 & 9269.8 & 498.3 & 1820.0 & 2392.7 &  1060.9  \\
HDFS & 11,167,740 & 46 & 1403.0 & 1123.3 & 4953.8 & 12070.0 &  836.7  \\
Spark & 16,075,117 & 236 & -- &  1593.8 & 8941.6 & 13931.9 & 1190.1 \\
Thunderbird & 16,601,745 & 1241 & 11807.5 & 2491.8 & 15503.2 & 26944.9 &  2913.4\\
\hline
Average & 3,601,187 & 249.1 & 1793.6 & 425.4 & 2293.8 & 4097.6 & 569.6 \\
\bottomrule
\end{tabular}
}
\end{table*}



==> bp/03-method-bp.tex <==
\newpage

\section{Method}



\subsection{Overview}

\jy{Put overview here, mainly two modules: query cache and LLM, then 3.2 query cache, 3.3 LLM with ICL}

\subsection{Framework of Log Parsing with LLM}

\zh{to add a brief overview}

\subsubsection{Query Cache}

Previous studies~\cite{x} indicate that the number of log templates is several orders of magnitude smaller than the number of log messages.
This is attributed to the fact that a single log statement can generate a multitude of log messages, each with distinct parameters, yet all belonging to the same log template.
For instance, the large-scale log dataset, LogPub~\cite{x}, from LogPAI~\cite{x}, contains over 50 million log messages in total.
However, the total number of log templates is less than 250.
This implies that the ratio of the number of log messages to the number of templates exceeds twenty thousand.
Such circumstance is even more pronounced in real-world production environments~\cite{x}.
\jy{this paragraph is the motivation for using cache in the framework, should be put in the overview; As in here, should introduce what is the function of the Cache itself (input, output, efficiency), why existing cache not work (e.g., directly use regex), so you propose a tree-based cache}

Motivated by this observation, we introduce a novel component, \ourtree into our framework.
Query cache stores the answers of the LLM, which can also be updated during runtime.
By utilizing \ourtree, we can diminish the frequency of querying the LLM, as it can avoid multiple LLM queries of log messages belonging to the same template.
This can be done by prioritizing the inspection of the cache to determine if the template for the current log message already exists.
Besides, the \ourtree can fix the answers of the LLM, thereby augmenting the consistency among the generated log templates.
This is vital for enhancing the accuracy of grouping log messages.

Although the LLM can correctly parse most logs with the assistance of ICL, its singular focus on the semantic information of individual logs may lead to the creation of erroneous templates, a consequence of neglecting the global information of the whole log data.
For example, when parse a log message \fixedwidth{``User root successfully login.''}, it is difficult to determine whether the \fixedwidth{``root''} is a parameter or not.
However, when considering this log message with other log messages (\eg \fixedwidth{``User user1 successfully login.''}), we can ascertain that \fixedwidth{``root''} and \fixedwidth{``user1''} are dynamic parameters, indicating the username.
To utilizing the global information, we propose an update mechanism for the \ourtree, which will be further introduced in Sec.~\ref{}, thus allowing \nm incorporating the capability of the LLM and the global information to enable accurate log parsing.\jy{oh! don't put this here}

Specifically, \nm employs a tree structure to serve as the \ourtree, storing the generated log templates of the LLM.
In the \ourtree, all log templates can be split into a list of tokens using delimiters, and these tokens are stored in the tree from top to bottom. 
Each intermediate node in the tree represents a token, with the \fixedwidth{``<*>''} denoting the wildcard token that can match any token.\jy{too detailed, only intuition is needed, for example, this sentence should appear in the matching step, not here}
The leaf nodes of the tree contain a unique log template, which corresponds to a string obtained by concatenating all tokens contained in all intermediate nodes on the unique path from the root node to the leaf node.
Fig.~\ref{x} demonstrates the tree of \ourtree which stores three log templates.
This tree structure allows for efficient storage and retrieval of log templates, as we can accomplish the retrieval process through a single traversal from the root to the leaf node, without the necessity to sequentially check each template.
Moreover, the tree structure can directly reflect the similarity among log templates, that is, log templates within the same subtree share a common prefix.
This can aid the update mechanism of the \ourtree, which will be further discussed in Sec.\ref{x}.


\subsubsection{Step1: Preprocessing}
\label{sec: step1-preprocessing}

Following previous works~\cite{x}, for each log, we first preprocess it to split different fileds of log message, such as timestamp, component, logging level and content.
Similar to other studies, our focus lies in parsing the content of each log message.
In contrast, our framework does not rely on manually defined regular expressions to preprocess part of parameters, as this approach is both domain-specific and labor-intensive.
After extract the content of log messages, we split each message into a series of tokens by delimiters.
The delimiters for tokenization include white-space and other special characters, such as \fixedwidth{``,''} and \fixedwidth{``=''}.
These tokens are solely utilized within the tree structure, implying that we do not employ tokenization when querying the LLM to parse log messages.
This ensures that the parsing results of our framework are not severely impacted by the choice of delimiters, which has been identified as a drawback of existing methods~\cite{x}.


\subsubsection{Step2: Cache Matching}
\label{sec: step2}

After tokenizing the content of each log message, we first check whether the template of this log message is already stored in \ourtree.
If it is, we can directly conclude the parsing process of this log message, thereby circumventing the duplicate queries of the LLM.\jy{this should show in the overview framework}

To determine whether a log message template has already been archived in \ourtree, a matching process is implemented to identify any log templates within \ourtree that perfectly correspond to the content of the log.
Fig~\ref{x} offers a visual representation of this matching process.
\ourtree may encompass numerous log templates, each of which corresponds to a path from the root to a leaf node within the tree.
Given a list of tokens from a log message, these tokens are read sequentially from the first to the last, with each being compared to nodes within the tree.
For the initial token, a search is conducted to ascertain its presence in the second layer of the tree, with the first layer being the empty root node.
If a match is found for the first token, the process continues with the second token and the children of the matched node.
This process is stopped once all tokens have been read.
If a leaf node is reached, the corresponding template is returned.
Otherwise, \fixedwidth{NONE} is returned to indicate a mismatch.
We will also return the templates of the leaf nodes within the subtree of current stop node.
These \textit{related templates} possess a prefix identical to this log message, indicating a degree of correlation.
It is important to note that \fixedwidth{``<*>''} within a template represents parameters of variable length, thus \fixedwidth{``<*>''} within the tree is permitted to match more than one token if no child node of \fixedwidth{``<*>''} matches the subsequent log token.
To prevent overly broad matching, a limit is also imposed on the maximum number of tokens that a single \fixedwidth{``<*>''} can match.


% if matched
If any log template is returned after the matching process, it signifies that the template for this particular log message is already stored in the \ourtree.
This could be attributed to a previous query to the LLM to generate this template while processing another log message associated with it.
Consequently, there is no necessity to query the LLM again, and the id of the leaf node can be recorded as its template id.
In some special cases, multiple successfully matched templates may be returned.
Consistent with previous research~\cite{jiang2023large}, the template with the longest constant parts is selected, as it can match more non \fixedwidth{``<*>''} characters, thereby increasing the likelihood of it being the template for this log message.


% In another situation
If no log template is matched in \ourtree, the templates within the subtree of the stop node are returned, comprise a list of related templates, \ie $[T_1, T_2, \cdots, T_n]$.
These related templates possess a portion of prefixes identical to the current log message, yet they fail to exactly match the entire log message.
This could potentially be attributed to the fact that during previous query processes, the LLM was only capable of parsing individual log messages, thereby failing to accurately identify parameters, resulting in the generation of overly specific templates.
Consequently, we record these potentially erroneous templates for subsequent steps.


\subsubsection{Step3: LLM Querying}

If the matching of templates in \ourtree failed, then we need to query the LLM to parse this single log message.
Leveraging the semantic comprehension and pre-training knowledge of LLMs, we can directly input the designed instruction and the original log message to the LLM.
Subsequently, the LLM will return the template of this log message following the instruction, denoted as $T_{a}$.
To enhance the performance of LLM in the task of log parsing, we have further devised the prompt to utilize the LLM's ICL capabilities, which will be elaborated upon in detail in Sec.~\ref{sec: LLM design}.
Upon querying the LLM, the log template generated in its answer, marked as $T_a$, will be extracted.

\subsubsection{Step4: Cache Updating}

When the LLM generates excessively specific templates, it could potentially result in the mismatch of log messages within the same template\jy{not clear, show examples}, thereby leading to additional queries and generate more templates.
To mitigate this problem, after get the newly generated log template $T_a$, we first discern whether $T_a$ could potentially belong to the same ground-truth template as any erroneous template in \ourtree.
Specifically, we calculate the similarities between $T_a$ and all related templates $T_1, T_2, \cdots, T_n$, since these related templates share the common prefix with the queried log message.
Given two templates $T_1$ and $T_2$, we split them into a list of tokens, denoted as $L_1$ and $L_2$.
Then, the similarity between $T_1$ and $T_2$ is defined as following:
\begin{equation*}
    Sim(T_1, T_2) = \frac{2 \times len(LCS(L_1, L_2))}{len(L_1) + len(L_2)}
\end{equation*}
We choose $T_b$ from all related templates, which exhibits the highest similarity with $T_a$.
If $Sim(T_a, T_b)$ exceeds the pre-defined threshold, we merge $T_a$ into $T_b$.
This is achieved by updating the $T_b$ in \ourtree, wherein the differing tokens are replaced with the \fixedwidth{``<*>''}.
In contrast, if the similarity is smaller than the threshold, the new template $T_a$ is simply added to \ourtree.
In this manner, \nm can dynamically modify the \ourtree, utilizing both the answers of the LLM and the global information of log data, thus enhancing the accuracy of the parsed templates.
Moreover, as \ourtree only retains the generated templates, and the number of these templates is considerably less than the log numbers, the overhead associated with cache updates is typically minimal.



\subsection{LLM module with ICL}
\label{sec: LLM design}
% draw a framework

As shown in Fig.~\cite{x}, in the LLM module of \nm, we introduce effective and efficient \textit{candidate sampling} and \textit{demonstration selection} algorithms to leverage the ICL capability of the LLM for log parsing.
In addition, we design a prompt format that incorporates ICL to query the LLM.
\jy{need an overview, you only mention the names of each component, this is unclear, you need to elaborate the overall running pipeline and the role of each component here.}

\subsubsection{Candidate Sampling}
\label{sec: candidate sampling}

A typical application of ICL in log parsing is first sample a candidate set of log messages.
These candidates should be diverse and representative, \ie they should cover as many characteristics in the whole log data as possible~\cite{x}.
These candidate logs should be manually labelled with its grountruth log template.
Moreover, the number of sampled candidates are significantly less than that needed for the training-based model in this few-shot scenarios (\eg 32-shot).
In real-world scenarios, this sampling step can be initially performed on the log data already generated by the system.
Then, it can be executed intermittently in an automated manner, thereby maintaining a dynamic candidate set that can adapt to the evolution of log data.
Therefore, the efficiency of the sampling process is essential in practical.

% In order to facilitate the efficient and effective sampling of demonstration candidates for ICL, we introduce a hierarchical clustering-based sampling algorithm.
To this end, we propose a hierarchical clustering-based sampling algorithm for ICL in log parsing.
First, we categorize the entirety of the log data into hierarchical clusters, utilizing token frequency and specific formats.
Then, we adopt a hierarchical quota distribution approach across the hierarchical clusters, assigning priorities in accordance with the size of each cluster.
This methodology offers two primary benefits.
Firstly, it ensures the diversity of the sampled candidates, thereby mitigating the potential bias in the sampling process that may arise from imbalanced template frequencies.
Secondly, it enables the sampled candidates to represent as many log messages as possible, thereby enhancing their representativeness.

The detailed algorithm is illustrated in Fig.~\cite{x}.
The first stage of our clustering procedure draws inspiration from preceding research~\cite{liu2019logzipIC,jiang2023large}, utilizing the top-K frequent tokens to group logs.
We employ the same delimiters used in Sec.\ref{sec: step1-preprocessing} to tokenize each log.
Subsequently, the frequencies of all tokens within the log data is calculated, exclude of stop words provided by the Scipy library~\cite{}.
For each log message, tokens with top-K frequencies are selected, which forms the basis for their categorization into different \textit{coarse-grained clusters}.
In other words, all log messages within the same coarse-grained clusters share the same top-K frequent tokens, indicating a degree of similarity.

However, simply utilizing the frequent tokens cannot adequately represent the characteristics of log message.
One primary reason is that it overlooks the special characters in log messages, namely, characters that are not alphabets, numerals, or white-space.
These special characteristics are also important to reflect the features of log messages.
Specifically, we define the set of special characters in a single log message as its \textit{special format}.
For instance, the special format of \fixedwidth{``Received block blk\_358 of size 6710 from /127.0.0.1''} is \fixedwidth{\{`\_',`.',`/'\}}.
Typically, log messages that originate from the same template share an identical special format.
This is attributed to the fact that the special characters in the constant parts (\ie the template) of a log are invariably identical, while those in the dynamic parts (\ie the parameter) are generally congruent.
Consider, for instance, the first parameter in the aforementioned log message, \fixedwidth{`blk\_358'}.
For other logs that share the same template, their first parameter might be \fixedwidth{`blk\_i'}, where \fixedwidth{i} represents a specific identifier.
Consequently, the first parameters of these logs share the same set of special characters, \ie \fixedwidth{`\_'}.
This suggests that the special format can encapsulate a portion of the logs' characteristics, given its potential to differentiate logs that belong to different templates.
Moreover, as identified in some previous studies~\cite{}, the variety of delimiters can significantly impact the performance of log parsers.
By integrating the special format to sample logs, it could potentially facilitate the LLM to adapt to various log message formats.

Therefore, the second stage involves the representativeness of the special format of log message.
% We employed token information for a preliminary coarse clustering in the first stage, yet this overlooked the special format information within the log.
We further divide each coarse-grained cluster according to the special formats of logs.
Through this method, we obtain \textit{fine-grained clusters}, wherein all log messages not only possess identical top-K frequent tokens but also share the same log format.


% After obtain these hierarchical clusters, we need to sample diverse and representative candidate logs from them.
We denote the number of coarse-grained clusters as $N_c$, and that of fine-grained clusters and $N_f$.
Recall that the design of the LLM module in \nm is intended to leverage the ICL capabilities of the LLM in few-shot scenarios.
This implies that the number of sampled candidates, $K_s$, is typically small, for instance, ranging from 16 to 128 in practical applications, which can decrease the burden of manual labeling.
Hence, in the majority of instances, the number of fine-grained clusters surpasses the number of sampled candidates, \ie $N_f > K_s$.
Therefore, we need to determine how to choose these candidates aiming to enhance both the diversity and representativeness.

To achieve this, we apply a hierarchical sampling strategy to these clusters.
Our principal idea is to distribute the quota of k candidates into more diverse and representative clusters through a hierarchical approach.
Initially, all coarse-grained clusters are arranged in descending order according to the number of logs they contain.
These sorted coarse-grained clusters are denoted as $C_1, C_2, \cdots, C_{N_c}$.
Moreover, within each coarse-grained cluster $C_i$, all fine-grained clusters are similarly arranged in descending order.
Then, the quota for $K_s$ candidates is distributed amongst the $N_c$ coarse-grained clusters, ensuring that cluster $C_i$ is allotted a quota of $S(C_i)$  , where:
\begin{equation*}
S(C_i) =
\begin{cases}
\lfloor \frac{K_s}{N_c} \rfloor + 1 &\quad\text{if } i \le (K_s \bmod N_c)\\
\lfloor \frac{K_s}{N_c} \rfloor &\quad\text{otherwise}\\
\end{cases}
\end{equation*}
On one hand, such a strategy ensures that the sampled candidates are drawn as evenly as possible from various clusters, thereby enhancing the diversity.
On the other hand, it also guarantees that in instances where an entirely equitable distribution is unattainable, clusters containing a greater number of logs are accorded higher priority, thereby augmenting the representativeness of the sampled candidates.
Once the quota for each coarse-grained cluster has been determined, it remains necessary to further distribute these quotas into the fine-grained clusters.
We utilize the same allocation strategy function $S$, to augment the diversity and representation of the sampled candidates.
As previously mentioned, in the majority of instances, $K_s$ is small, hence the quota allocation for each fine-grained cluster is typically minimal(\eg ranging from zero to two).
Consequently, we finally randomly select assigned number of candidates within each fine-grained cluster to ensure the high efficiency.



\subsubsection{Demonstration Selection}
\label{sec: demonstration selection}

% For each log to be queried, it is then necessary to select several demonstration examples from the candidate set.
For each log to be queried, we need to select $k$ demonstration examples from the $K_s$ candidates sampled in Sec.~\ref{sec: candidate sampling}.
These demonstration logs should bear similarity to the log in the query, enabling the LLM to utilize the patterns and semantics learnt from the examples to parse the queried log~\cite{x}.

In \nm, we adopt k-Nearest Neighbors (kNN), a simple yet effective algorithm to select the demonstration examples of each queried log.
In specific, for each queried log, denoted as $l$, we initially compute the similarities between it and all logs within the candidates sets, \ie $sim(l, s_i)$, $i \in [1, K_s]$.
In order to enhance the reflective capacity of the similarity function, $sim$, regarding the degree of resemblance between the characteristics of two logs, we combine the similarity of tokens and special format of log message.
In detail, for the log message $l$, we split it by delimiters to get a list of tokens, which are subsequently transmuted into a set of tokens.
Then, we extract the special characters within $l$, yielding another set of special characters.
We merge these two sets, thereby obtaining the \textit{characteristic set}, $C(l)$, of this log message.
Based on this, we can determine the value of similarity function of two log messages by calculating the Jaccard similarity~\cite{} of their characteristic sets, \ie $sim(l_1, l_2) = \frac{|C(l_1) \ \cap \ C(l_2)|}{|C(l_1) \ \cup \ C(l_2)|}$.
% Such definition of similarity between logs can comprehensively reflect the characteristics of logs 
After computed all similarities, we select the logs from the candidate sets that exhibit the top-$k$ highest similarities.
These logs, characterized by similar tokens and special characters to the queried log, are instrumental in aiding the LLM to comprehend the semantics and formats embedded within them.


\subsubsection{Prompt Design}

% As discussed in Sec.~\ref{sec: LLM-ICL}, ICL can assist the LLM in learning system-specific characteristics, thereby enhancing its capability to accurately parse each log message for diverse log data.
Following previous work~\cite{xu2023prompting,le2023evaluation}, we design and use the prompt format, as depicted in Fig.~\ref{x}, to query the LLM to generate log template for a individual log.
The prompt encompasses the following three parts.
\jy{the figure should clearly show how the prompt looks like, using concrete examples, also show the model output}
\begin{enumerate}[leftmargin=*, topsep=0pt]
    \item \textit{Instruction.}
    \citet{le2023evaluation} have identified that different instructions can influence the performance of LLMs in log parsing.
    Consequently, we adopt the instruction comprising four sentences, briefly introducing the task, the concept of log parsing, and the formats of both input and output.
    This prompt can help LLMs to quickly understand the demand of log parsing, thus improve their effectiveness in this downstream task.
    \item \textit{Demonstration Examples.}
    Subsequently, we integrate several demonstration examples, selected following the algorithm in Sec.~\ref{sec: demonstration selection}, into the prompt.
    Each example includes a pair of a log message and its corresponding log template.
    In addition, recent work~\cite{} has pinpointed that LLMs with ICL are more prone to the inductive bias of the examples that are closer to the query.
    Therefore, we arrange the demonstration examples in \textit{ascending order} of similarity to the queried log, \ie those of higher similarities closer to the queried log.
    This is based on the intuition that examples with higher similarity may encompass more information pertinent to parsing the queried log.
    \item \textit{Queried Log.}
    Last, we present the content of log message to enable the LLM parse it and generate its template.
    Guided by the instruction and demonstration examples, the LLM can accurately answer the log template of the queried log in the prompt, adhering to the correct format.
\end{enumerate}





\newpage







% The definition of a single log message's characteristics is crucial for both the sampling and selection stages.
% Some existing studies~\cite{x} define the similarity between two log messages as the similarity between their respective token lists.
% In specific, these logs are tokenized using particular delimiters, and then a certain similarity function, such as the Jaccard similarity~\cite{x}, is employed to ascertain their degree of similarity.
% However, 


% We highlight that these special characters play a significant role in representing the characteristics of log messages.
% Furthermore, 


% The definition of a single log message's characteristics is crucial for both the sampling and selection stages.
% Some existing studies~\cite{x} define the similarity between two log messages as the similarity between their respective token lists.
% In specific, these logs are tokenized using particular delimiters, and then a certain similarity function, such as the Jaccard similarity~\cite{x}, is employed to ascertain their degree of similarity.
% However, these methods overlook the special characters in log messages, namely, characters that are not alphabets, numerals, or white-space.

% \subsubsection{Special format of log}
% \label{sec: special format of log}
% We are the first to highlight that these special characters play a significant role in representing the characteristics of log messages.
% Furthermore, we define the set of special characters in a single log message as its \textit{special format}.
% For instance, the special format of \fixedwidth{``Received block blk\_358 of size 6710 from /127.0.0.1''} is \fixedwidth{\{`\_',`.',`/'\}}.
% Typically, log messages that originate from the same template share an identical special format.
% This is attributed to the fact that the special characters in the constant parts (\ie the template) of a log are invariably identical, while those in the dynamic parts (\ie the parameter) are generally congruent.
% Consider, for instance, the first parameter in the aforementioned log message, \fixedwidth{`blk\_358'}.
% For other logs that share the same template, their first parameter might be \fixedwidth{`blk\_i'}, where \fixedwidth{i} represents a specific identifier.
% Consequently, the first parameters of these logs share the same set of special characters, \ie \fixedwidth{`\_'}.
% This suggests that the special format can encapsulate a portion of the logs' characteristics, given its potential to differentiate logs that belong to different templates.
% Moreover, as identified in some previous studies~\cite{}, the variety of delimiters can significantly impact the performance of log parsers.
% By integrating the special format to sample logs, it could potentially facilitate the LLM to adapt to various log message formats.



